Nano-EmoX: Unifying Multimodal Emotional Intelligence from Perception to Empathy

The development of affective multimodal language models (MLMs) has long been constrained by a gap between low-level perception and high-level interaction, leading to fragmented affective capabilities and limited generalization. To bridge this gap, we propose a cognitively inspired three-level hierarchy that organizes affective tasks according to their cognitive depth-perception, understanding, and interaction-and provides a unified conceptual foundation for advancing affective modeling. Guided by this hierarchy, we introduce Nano-EmoX, a small-scale multitask MLM, and P2E (Perception-to-Empathy), a curriculum-based training framework. Nano-EmoX integrates a suite of omni-modal encoders, including an enhanced facial encoder and a fusion encoder, to capture key multimodal affective cues and improve cross-task transferability. The outputs are projected into a unified language space via heterogeneous adapters, empowering a lightweight language model to tackle diverse affective tasks. Concurrently, P2E progressively cultivates emotional intelligence by aligning rapid perception with chain-of-thought-driven empathy. To the best of our knowledge, Nano-EmoX is the first compact MLM (2.2B) to unify six core affective tasks across all three hierarchy levels, achieving state-of-the-art or highly competitive performance across multiple benchmarks, demonstrating excellent efficiency and generalization. The code is available at https://github.com/waHAHJIAHAO/Nano-EmoX.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}
To advance human-centric AI, systems must evolve beyond simple emotion perception toward a holistic emotional intelligence—a unified continuum from perception to interaction—as demanded by applications ranging from companionship to therapy. However, the current landscape of affective computing is a vast and fragmented collection of tasks, lacking a coherent structure to guide systematic progress or assess a model's true emotional maturity.

To bring order and clarity to this field, we posit a conceptual hierarchy that organizes affective tasks into a three-level hierarchy based on increasing cognitive depth. This hierarchy reflects a natural progression from sensation to reason to action. As described in \cref{fig:task hierarchy}, it begins at the foundational level of perception, which involves the direct recognition of raw emotional cues in tasks like multimodal emotion recognition. Then it ascends to the more complex level of understanding, which requires deeper cognitive processing to infer causality and intent in tasks such as emotion reason inference and intent recognition. The hierarchy culminates in the highest stratum, emotional interaction, which demands proactive, generative, and empathetic engagement, as exemplified by empathic response generation.
% Early research in affective computing progressed from unimodal approaches in text \cite{sabour2022cem,plaza2021multi}, audio \cite{cai2021speech,li2019attentive} and vision \cite{hallmen2024unimodal,savchenko2021facial} to more sophisticated multimodal frameworks \cite{peng2024carat,akhtar2019multi}, driven by the inherently cross-modal nature of human emotion. While these frameworks demonstrated the value of multitask learning, they often struggled with task generalization.
%--------------------------task hierarchy fig---------------------------------
\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{images/task_hierarchy.pdf}
    \caption{Affective tasks can be categorized into a three level hierarchy based on their complexity, where mastery of higher-level tasks necessitates a more profound emotional cognition. Please see the appendix for specific task definitions.}
    \label{fig:task hierarchy}
\end{figure}
%----------------------------------------------------------------

Viewing the field through this hierarchical lens illuminates its historical trajectory. Early research, from unimodal \cite{sabour2022cem,plaza2021multi,cai2021speech,li2019attentive,hallmen2024unimodal,savchenko2021facial} to multimodal pipelines \cite{peng2024carat,akhtar2019multi}, primarily targeted challenges within the perception and understanding level. The advent of Large Language Models (LLMs) \cite{fei-etal-2023-reasoning,wu2023improving,liu2024emollms} and Multimodal Language Models (MLMs) \cite{yang2024emollm,xie2024emovit,huang2025emotion,cheng2024emotion,lian2025affectgpt,yang2025omni,zhao2025r1} catalyzed a significant shift, enabling models to master analytical tasks at the understanding level, and has recently culminated in pioneering forays into the interaction stratum \cite{zhang2025towards,liu2024speak}.

% A paradigm shift occurred with the advent of Large Language Models (LLMs), whose vast prior knowledge and inferential capabilities led to remarkable success in text-based affective tasks \cite{fei-etal-2023-reasoning,wu2023improving,liu2024emollms}. The subsequent emergence of Multimodal Language Models (MLMs) marked a critical breakthrough. By synergizing powerful encoders with curated datasets \cite{yang2024emollm,xie2024emovit,huang2025emotion,cheng2024emotion,lian2025affectgpt,yang2025omni,zhou2025llm}, MLMs began to master a spectrum of complex analytical tasks, including Multimodal Emotion Recognition (MER), Reasoning (ERI) and Intent Recognition (MIR). This paradigm's efficacy was rapidly validated on unified benchmarks like MMLA \cite{zhang2025can}, propelling the research frontier beyond passive analysis toward active interaction. This culminated in pioneering generative tasks such as multimodal Empathic Response Generation (ERG) \cite{zhang2025towards,liu2024speak}.

%--------------------------compare tab-------------------------------------
\begin{table}[t]
\centering
\caption{Comparison with representative LLM-Based methods under different task settings, our method unifies six core affective tasks with a smaller parameter scale.}
\label{tab:cap compare}
\resizebox{\linewidth}{!}{ 
\renewcommand{\arraystretch}{1.3} 
\begin{tabular}{>{\large}c>{\large}c>{\large}cccccccc}   % 所有列均居中对齐，消除左对齐导致的空白
\toprule
% 表头文字居中，旋转标题以中心为锚点，减少偏移
\textbf{Models} & \textbf{Scale} & \textbf{Hierarchy} & 
\rotatebox[origin=c]{45}{\textbf{MSA}} & \rotatebox[origin=c]{45}{\textbf{MER}} & 
\rotatebox[origin=c]{45}{\textbf{OV-MER}} & \rotatebox[origin=c]{45}{\textbf{ERI}} & 
\rotatebox[origin=c]{45}{\textbf{MIR}} & \rotatebox[origin=c]{45}{\textbf{ERG}} \\
\midrule
EmoLLMs \cite{liu2024emollms} & 7B & level 1 & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} &  \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} \\
Emotion-LLaMA \cite{cheng2024emotion} & 8.3B & level 2 & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} \\
Omni-Emotion \cite{yang2025omni} & 8.6B & level 2 & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} \\
LGSRR \cite{zhou2025llm} & 7.1B & level 2 & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} \\
E3RG \cite{lin2025e3rg} & 7B & level 3 & \textcolor{red}{×} &\textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{green}{\checkmark} \\
Empatheia \cite{zhang2025towards} & 8B & level 1\&3 & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{green}{\checkmark} \\
EmoVerse \cite{li2024emoverse} & 4/8B & level 1\&2 & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} \\
AffectGPT \cite{lian2025affectgpt} & 7.8B & level 1\&2 & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} \\
Emotion-Qwen \cite{huang2025emotion} & 7.5B & level 1\&2 & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} \\
SMES \cite{chu2025towards} & 7.1B & level 1\&3 & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{red}{×} & \textcolor{green}{\checkmark} \\
R1-Omni \cite{zhao2025r1} & 2.1B & level 1\&2 & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{green}{\checkmark} & \textcolor{red}{×} & \textcolor{red}{×} \\
\midrule
\textbf{Our Nano EmoX} & 2.2B & level 1$ \sim $3 & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} & \textcolor{green}{\checkmark} \\
\bottomrule
\end{tabular}
}
\end{table}

%--------------------------compare tab-------------------------------------
Nevertheless, this upward progression reveals a fundamental schism: current models typically operate as level-specialists, excelling at tasks within one cognitive stratum but failing to integrate knowledge across the hierarchy \cite{liu2024emollms,cheng2024emotion,yang2025omni,zhou2025llm,lin2025e3rg}. The development of a single unified agent that spans the entire perception to interaction continuum remains a major open challenge. 

First, \textbf{suboptimal fusion:} existing fusion mechanisms struggle to adapt to the diverse feature requirements of different cognitive strata, limiting the model's ability to generalize across levels. Second, \textbf{fragmented capabilities:} as shown in \cref{tab:cap compare}, the knowledge currently mastered by the model is isolated. Without learning the deep connections between perceiving an emotion and reasoning about its cause, models lack true comprehension, making the deployment of multiple specialist models an impractical and inefficient necessity. Finally, \textbf{resource intensity:} the intensive computing and data resources required for training and inference by most LLM-based methods hinder the widespread application of a comprehensive affective agent in the real world.
% Despite such rapid progress, the path toward practical and truly general-purpose affective AI remains hindered by three fundamental challenges. First, current methods rely solely on simple attention or the fusion mechanisms of LLMs, thus fail to capture complementary information with optimal contribution weights tailored to diverse task requirements, this limits the model’s cross-task generalization ability. Second, as illustrated in \cref{tab:cap compare}, the complexity and heterogeneity of emotional tasks lead to fragmented capabilities, prior models fail to learn deep hierarchical connections between tasks or unify cross-hierarchical emotional knowledge into a single model, Deploying multiple models to perform multiple tasks is impractical and computationally inefficient. Finally, the prohibitive parameter scales of most state-of-the-art (SOTA) methods incur exorbitant research and deployment costs, creating an urgent need for more parameter-efficient solutions for real-world applications.

To address the limitations, we introduce \textbf{Nano EmoX}, a compact, hybrid-inference MLM that unifies six core affective tasks: multimodal sentiment analysis (MSA), multimodal emotion recognition (MER), Open Vocabulary MER (OV-MER), multimodal intention recognition (MIR), emotion reason inference (ERI), empathetic response generation (ERG). Specifically, Nano EmoX integrates Omni-modal inputs. Beyond capturing generic visual and acoustic cues, our model explicitly models fine-grained facial affective signals and simultaneously implements an early, hierarchical and dynamic speech-visual feature fusion. Following a dimensional alignment step performed by heterogeneous adapters, the language model (LM) proceeds to tackle all downstream tasks.

Building on this, we propose \textbf{the P2E (Perception-to-Empathy) framework}, designed to efficiently unlock the full potential of the model in emotional intelligence. The core of this framework lies in a meticulously designed data curriculum and a progressive training procedure. Initially, P2E enables the model to establish foundational perception and acquire multimodal fusion knowledge. Subsequently, it cultivates advanced capabilities in affective reasoning and empathy. Experimental results validate the effectiveness of the P2E framwork for learning multilevel tasks. Our contributions are summarized as follows:
\begin{itemize}
    \item \textbf{A unifying and original perspective.} We propose a \emph{novel three-level cognitive hierarchy}—perception, understanding, and interaction—that organizes affective tasks according to their cognitive depth. This framework, first introduced in our work, provides a unified and logically progressive taxonomy for affective modeling, offering a new conceptual foundation for future research in emotional intelligence.
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%
    %%    一个句子里不要有两个重复的词 We xxxxx a hierarchical xxxxx hierarchy xxxxxx
    %%   contributions要突出创新逻辑，我再这一点里也加入了原创的3个levels你看看合不合适
    %%
    %%    供你参考：
    %%    \item \textbf{A unifying and original perspective.} We propose a \emph{novel three-level cognitive hierarchy}—perception, understanding, and interaction—that organizes affective tasks according to their cognitive depth. This framework, first introduced in our work, provides a unified and logically progressive taxonomy for affective modeling, offering a new conceptual foundation for future research in emotional intelligence.
    %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \item \textbf{A smaller yet stronger MLM.} We present Nano EmoX, a omni-modal, small-scale MLM that integrates a dedicated facial encoder and a gated hierarchical fusion encoder for dynamic audio–visual alignment. This design enables fine-grained affect modeling and strong cross-task generalization at deployable scale.
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%
    %%    强调模型结构创新
    %%     omni-modal 这个词别的人也是这么用的吗？还是multimodal？
    %%
    %%    供你参考：
    %%    \item \textbf{A smaller yet stronger MLM.} We present Nano EmoX, a compact 2.2B-parameter multimodal language model that integrates a dedicated facial encoder and a gated hierarchical fusion encoder for dynamic audio–visual alignment. This design enables fine-grained affect modeling and strong cross-task generalization at deployable scale.
    %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \item \textbf{An affective task fine-tuning framework.} We introduce the P2E, a fine-tuning framework designed for low-compute resource settings, which efficiently imparts multilevel affective knowledge through a progressive curriculum design.
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%
    %%    “A affective” → 应为 “An affective”。
    %%
    %%    供你参考：
    %%    \item \textbf{An affective task fine-tuning framework.} We propose P2E (Perception-to-Empathy), a curriculum-based fine-tuning framework that progressively cultivates multilevel affective understanding—from rapid perceptual recognition to empathetic reasoning—while maintaining high efficiency under limited computational resources.
    %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    \item \textbf{State-of-the-art performance.} To the best of our knowledge, Nano EmoX is the first compact MLM to unify six core affective tasks across all hierarchy levels. It achieves state-of-the-art or highly competitive performance on multiple benchmarks, demonstrating an effective balance between model capacity, generalization, and deployability.
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%
    %%    “State-of-The-Art” 应改为 “State-of-the-art”。
    %%    表述太长、重复。应强调创新性
    %%    供你参考：
    %%    \item \textbf{State-of-the-art performance.} To the best of our knowledge, Nano EmoX is the first compact model to unify six core affective tasks across all hierarchy levels. It achieves state-of-the-art or highly competitive performance on multiple benchmarks, demonstrating an effective balance between model capacity, generalization, and deployability.
    %%
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{itemize}

% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.

%-------------------------------Nano Emox pipeline fig------------------------------------------
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{images/EmoX-pipeline.pdf}
  \caption{The architecture of the Nano EmoX. The visual branch extracts general visual emotional cues, the facial branch is responsible for modeling fine-grained facial details, the voice branch captures voice emotional cues. To balance the contribution of each modality, the fusion branch integrates key emotional cues from the audio-visual modalities and extracts complementary information. The language model integrates multimodal information and performs multitask emotion recognition.}
  \label{fig:model overview}
\end{figure*}
%-------------------------------Nano Emox pipeline fig------------------------------------------

==> sec/2_related.tex <==
\section{Related Work}
\label{sec:related work}

\subsection{Multimodal Language Model}
The advent of MLMs, exemplified by models such as SALMONN \cite{tang2023salmonn}, Video-LLaMA \cite{zhang2023video}, Qwen2.5-Omni \cite{xu2025qwen2} and MiniCPM V-2.6 \cite{hu2024minicpm}, has revolutionized the field by deeply integrating pre-trained modality encoders with LLMs. This fusion has led to remarkable advancements in tasks like visual question answering and audio-language understanding.

Despite the impressive general capabilities exhibited by these MLMs, a significant deficiency in their emotional intelligence persists. Comprehensive benchmarks like EmoBench \cite{sabour2024emobench}, MMLA\cite{zhang2025can} and EmoBench-M \cite{huemobench} have systematically evaluated prominent open-source and proprietary models, including BLIP 2 \cite{li2023blip}, InternLM 2.5 \cite{wu2024internlm2}, GPT-4 \cite{achiam2023gpt} and Gemini-2.0-Flash \cite{comanici2025gemini}. The findings consistently reveal a substantial gap between the emotional comprehension abilities of these state-of-the-art models and human performance.

This disparity has fueled a recent surge in research dedicated to specializing MLMs for emotional domains, as seen in works like EmoVIT \cite{xie2024emovit} and Emotion-Qwen \cite{huang2025emotion}. More recent investigations, such as Emotin-LLaMA \cite{cheng2024emotion} and AffectGPT \cite{lian2025affectgpt}, have further incorporated audio and video features to achieve explainable emotion recognition and causal reasoning. To enhance reasoning quality, some studies have begun exploring reinforcement learning method, with R1-Omni \cite{zhao2025r1} exemplifying this by training an explainable, smaller scale MLM. Concurrently, cutting-edge research in empathetic response generation is also underway \cite{zhang2025towards,liu2024speak}, with the aim of constructing conversational agents with more human-like qualities. However, these works merely rely on static fusion mechanism within the LM, fail to dynamically fuse speech-visual modal signals in a task-aware manner and do not focus on modeling facial visual signals that can stably express emotions.

To address this limitation, we propose \textbf{Nano EmoX}, including a fusion encoder and a facial encoder. Ablation studies demonstrate that our 2.2B model enables better adaptive modeling of multimodal signals, thereby enhancing task processing performance.

\subsection{Multitask Learning for Emotion-centric MLM}
The advent of the Transformer architecture \cite{vaswani2017attention} and its outstanding generalization ability have profoundly advanced the multitask learning research paradigm and stimulated the development of large scale vertical emotion models for handling multiple tasks. For instance, EmoLLMs \cite{liu2024emollms} attempt to optimize and unify five text emotion tasks through instruction fine-tuning (IF). In the multimodal field, Emotion-LLama \cite{cheng2024emotion} and AffectGPT \cite{lian2025affectgpt} adopt a joint training approach to train models to master the skills of emotion recognition and emotion reason inference. Omni-Emotion \cite{yang2025omni} uses pre-trained and fine-tuned LMs to enhance emotion processing capabilities while maintaining general visual understanding abilities. EmoVerse \cite{li2024emoverse} proposed the M2SE IF strategy, which demonstrates the potential to improve the processing ability of emotional multitasking of the model through training strategies.

Nevertheless, prior works has been confined to training models to master knowledge at a single level, such as emotion understanding. In contrast, the \textbf{P2E training framework} facilitates the model in learning capabilities to process emotional tasks that span from perception to empathy. 

==> sec/3_method.tex <==
\section{Methodology}
\label{sec:methodology}

\subsection{Architecture of Nano EmoX}
\label{sec:nano_emox}
Nano EmoX is a compact hybrid-reasoning, multitasking and multimodal MLM for emotion tasks. As depicted in \cref{fig:model overview}, it consists of four modal branches and a language backbone.

\textbf{Scene visual perception branch:} To perceive generic visual signals, we employ a pre-trained visual encoder on large-scale data to process video frames $x_v\in\mathbb{R}^{3 \times H \times W}$, yielding general-purpose visual emotion embeddings: $ E_v$.
% \begin{equation}
%     E_v = f_{\text{CLIP}}(x_v)
%     \label{eq:visual_encoding}
% \end{equation}
Here, $H$ and $W$ denote the frame length and the feature dimension, respectively. 

Given that reducing the scale of LMs decreases the number of neurons agnostic to the modality~\cite{schwettmann2023multimodal}, we posit that incorporating a resampling network upstream of LM can alleviate this problem and improve expressiveness. Thus, the visual branch leverages a two-layer Q-Former~\cite{li2023blip} to resample visual tokens $T_v \in \mathbb{R}^{T_v \times D_v}$, enriching emotional representation. In this notation, $T_v$ and $D_v$ represent the length and dimension of the visual token, respectively.

\textbf{Speech perception branch:} To extract high-quality acoustic features, such as prosody and pitch, we employ a pre-trained speech encoder to process the audio frames $x_a \in \mathbb{R}^{ T_{a1} \times D_{a1}}$ (sampled at 1.6 kHz), obtaining speech emotion embeddings: $E_a$.
% \begin{equation}
%     E_a = f_{\text{HuBERT}}(x_a)
%     \label{eq:speech_encoding}
% \end{equation}
Here, $T_{a1}$ and $D_{a1}$ denote the length and Mel spectrogram dimension of the audio frames, respectively.

Similarly, the speech branch employs a two-layer Q-Former to extract fine-grained speech tokens $T_a \in \mathbb{R}^{T_{a2} \times D_{a2}}$, where $T_{a2}$ and $D_{a2}$ denote the length and dimension of the token, respectively.

\textbf{Facial modeling branch:} Since facial expressions are crucial cues for conveying visual emotional features, modeling fine-grained facial representations is vital to enhancing the emotion perception capability of Nano EmoX. 

The FaceXFormer~\cite{narayan2024facexformer} encoder excels at extracting fine-grained, identity-invariant facial representations. We enhanced the encoder by shifting its processing paradigm from the original image-level processing to frame sequence processing. Specifically, we employ a facial encoder to process video frames $x_v$ for the extraction of multi-scale features $E_f$. Subsequently, Time Attention Pooling (TAP) is applied to halve the length of the feature sequence, enabling the capture of key facial features for emotion expression $E_f^c$. The core computation of TAP is formalized as:
\begin{equation}
    E_f^c = \text{CrossAttention}(Q, E_f^K, E_f^V)
    \label{eq:TAP}
\end{equation}
where $Q \in \mathbb{R}^{T_{f1} \times D_f}$ denotes learnable query vectors, $T_{f1}$ is the compressed sequence length, $E_f^K$ and $E_f^V$ are key/value features projected from the face embedding $E_f$.

Subsequently, a two fully connected layers network with GeLU~\cite{hendrycks2016gaussian} performs dimension alignment to the LM, generates the face token $T_f \in \mathbb{R}^{T_f \times D_f}$, where $T_f$ and $D_f$ denote the length and feature dimension of the token, respectively. For detailed network specifications, refer to the appendix.

\textbf{Cross-modal hierarchical fusion branch:} To enhance the model's multitask capabilities, we introduce a fusion encoder, which comprising three experts with independent weights and a gating network. Inspired by~\cite{zhao2024improving, chen2024finecliper, pastor2022cross, ding2023learning} and recognizing the pivotal role of speech features in emotion-related tasks, as well as the benefits of multiscale semantic information, we devise a unique fusion expert.

This expert employs speech features as queries to guide visual features through cross-modal cross-attention. Specifically, the encoder extracts intermediate features from layers 16, 18, 22 of the speech encoder and from layers 12, 16, 22 of the visual encoder. These features are then hierarchically paired from lower to higher levels and fed into the three corresponding fusion experts to generate fused representations $E_{mf}^i$. The gating network, consisting of a two-layer fully connected network with GeLU, dynamically routes the output of each expert by adjusting their contributions $G_i$ based on the specific feature demands of each task. The gating network process is formulated as follows:
\begin{equation}
    G_1, G_2, G_3 = f_{\text{gate}}(\text{Concat}(E_{mf}^1, E_{mf}^2, E_{mf}^3))
    \label{eq:gate_network_weight}
\end{equation}
\begin{equation}
    E_{mf} = G_1 \odot E_{mf}^1 + G_2 \odot E_{mf}^2 + G_3 \odot E_{mf}^3
    \label{eq:gate_network_add_weight}
\end{equation}
here, $E_{mf}$ represents the final fusion embedding, $f_{\text{gate}}$ represents the gated network processing

Finally, an adapter network projects the dimensionality of the fused features to align with that of the LM, generating the fusion tokens $T_f \in \mathbb{R}^{T_h \times D_h}$, where $T_h$ and $D_h$ denote the length and feature dimension of the token, respectively.
Using its hierarchical structure and dynamic gating mechanism, the fusion encoder is able to learn robust mappings between tasks and modalities. Please refer to the appendix.

\textbf{The core of language processing:} We use the Qwen2.5~\cite{qwen2025qwen25technicalreport} tokenizer to process prompt templates, dialogues, subtitles and other text to generate text tokens. small-scale LM then integrates tokens from all modalities to accomplish various downstream emotion tasks. 

% \subsection{Task Hierarchy}
% \label{sec:task hierarchy}
% To implement our P2E framework, \cref{fig:P2E} illustrates the hierarchical organization of emotional multitasks. Specifically, the foundational perception layer establishes an initial awareness of emotions, encompassing tasks such as MSA, MER, and OV-MER. The cognitive and causal reasoning layer serves as a crucial bridge to higher-level emotional interaction; it requires the model to deepen its comprehension of emotions, infer causal relationships among emotional states, and recognize the social intentions of individuals, as exemplified by tasks such as ERI and MIR. Building upon these two foundational layers, the generative empathy layer enables the model to produce empathetic responses during interactions with users, such as the ERG task.

% \subsubsection{Data Curation}
% To acquire fine-grained facial feature data, we selected the CAER~\cite{lee2019context} and FERV39K~\cite{wang2022ferv39k} datasets, which together provide high-quality facial expression videos in a diverse range of emotionally rich scenarios. To learn the correlation between vocal prosody and emotional states, we incorporated CREMA-D~\cite{cao2014crema} and M3ED~\cite{zhao2022m3ed}, whose multiturn conversational data contain a wealth of natural intonation and pitch variations. For the OV-MER task, the MER-Caption+~\cite{lian2025affectgpt} dataset was selected as a cornerstone, owing to its large scale and inherent open vocabulary characteristics.

% For the ERI task, we employed both the MER-Caption+~\cite{lian2025affectgpt} dataset and the meticulously annotated MERR-Fine~\cite{cheng2024emotion} to enhance the explanatory capabilities of the modal. We used the MIntRec~\cite{MIntRec} and MIntRec2.0~\cite{zhang2024mintrec} datasets to For the MIR, which are specifically designed for this task in conversational contexts, guiding the model to recognize fine-grained social goals and attitudes.

% For the ERG task, we structured the AvaMERG~\cite{zhang2025towards} into a turn-based format, preserving the conversation history as context:$(Q_1^t,R_1^t),(Q_2^t,R_2^t),\dots$, where $Q_i^t$ is the user's textual query and $R_i^t$ is the model's past textual response. By structuring the data such that the current user input $(Q_n^t,Q_n^v,Q_n^a)$ serves as the query and the corresponding response is $R_n^t$ the generation target, the dataset simultaneously supports MER and ERG. Here, $Q_n^t$ represents the textual input,the $Q_n^v$,$Q_n^a$ visual/acoustic query,and $R_n^t$ the model's target textual response. 

%-------------------------------------------------------------------------
\subsection{The P2E Training Framework}
%-------------------------------------------------------------------------
\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{images/P2E.pdf}
  \caption{The P2E framework consists of a three phase instruction fine-tuning process. Phase 1 focuses on the MER task. To ensure a smooth learning curve, phase 2 builds upon this foundation by incorporating the MIR task. Finally, phase 3 revisits prior knowledge and integrates a diverse set of multi-level complex tasks, governed by a predefined data mixture ratio.}
  \label{fig:P2E}
\end{figure*}
%-------------------------------------------------------------------------
As shown in \cref{fig:P2E}, the P2E framework is a three-phase training curriculum, each phase following the law of cognitive development from shallow to deep. Specifically, the first phase focuses on basic emotion recognition, the second phase introduces multimodal fusion and contextual understanding and the third phase emphasizes OV-MER, ERI and ERG, ensuring effective transfer and integration of knowledge across phases. For the prompt word template used in task training and more details, refer to the appendix. We skipped training the MSA task because MSA knowledge could also be acquired by learning from other task models.

To adapt to different task formats, we use identifiers to distinguish different tasks in the instruction template (see appendix for details). The entire multitask training process is unified under a single objective: optimizing the maximum likelihood estimation (MLE) of model parameters $\theta$ across all modalities, which can be formalized as the following formula:
\begin{equation}
    \theta^{MLE} = \arg\max_{\theta \in \Theta} \sum \log P\left(Y \mid T; \theta\right)
    \label{eq:MLE_optimization}
\end{equation}
where $T$ represents the tokenized representation of each modality, $Y$ is the target output. The P2E framework achieves this goal through three carefully designed phases:

\textbf{Phase1: Foundational Modality Alignment:} We first establish a robust unimodal foundation (see \cref{fig:P2E}, Phase 1). Training is concentrated on the modality-specific adapters to align the feature spaces of each encoder with the LM's embedding space, while the rest of modules remain frozen. Specifically, visual and facial adapters are jointly trained on FERV39K~\cite{wang2022ferv39k} and CAER~\cite{lee2019context} to learn diverse visual-language knowledge and fine-grained facial cues. Concurrently, the speech adapter is trained on CREMA-D~\cite{cao2014crema} and M3ED~\cite{zhao2022m3ed} to capture emotional acoustic knowledge. 

\textbf{Phase2: Cross-modal Fusion Pre-training:} we posit that MIR task serves as a natural bridge between basic perception and higher-order reasoning, compelling the model to synthesize multimodal cues to infer social goals (see \cref{fig:P2E}, Phase 2). we use the MIntRec~\cite{MIntRec} and MIntRec2.0~\cite{zhang2024mintrec} datasets to facilitate the learning of effective multimodal integration. This phase activates and trains the fusion encoder while continuing to train all modality adapters; the remaining components stay frozen. For models without a fusion encoder architecture, this phase is retained to continue joint training of adapters in each branch.

\textbf{Phase3: Multitask Instruction Tuning:} This phase aims to cultivate synergy across tasks, from deepening fine-grained perception (OV-MER) to inspiring high-level empathy (see \cref{fig:P2E}, Phase 3). We fine-tune the fusion encoder and all adapters on a carefully curated data curriculum and activate a Low-Rank Adaptation (LoRA) module for the LM. The data sampling ratio is set to MER: OV-MER: MIR: ERI: ERG = 18: 28: 5: 31: 18 to fully unleash the model's potential.

For the OV-MER task, we select the MER-Caption+~\cite{lian2025affectgpt} dataset to train the model to capture fine-grained, multi-label emotional perception capabilities. For the ERI task, we employ MER-Caption+ along with the meticulously annotated MERR-Fine~\cite{cheng2024emotion} dataset to enhance the model's explanatory and reasoning abilities.

For the ERG task, we structure AvaMERG~\cite{zhang2025towards} into a turn-based format, preserving the dialogue history as context: \((Q_1^t, R_1^t), (Q_2^t, R_2^t), \dots\), where \(Q_i^t\) is the user's textual query and \(R_i^t\) is the model's previous textual response. By structuring the data in this way, the current user input \((Q_n^t, Q_n^v, Q_n^a)\) serves as the query, the corresponding response \(R_n^t\) is the generation target. Here, \(Q_n^t\) represents the textual input, \(Q_n^v\) and \(Q_n^a\) represent the visual and audio queries, respectively, \(R_n^t\) represents the model's target textual response. 

Subsequently, we draw on~\cite{zhang2025towards} to guide the model to first consider dialogue scenario, the speaker’s emotion and response goal, thereby generating higher quality empathetic responses. The thinking process is wrapped up in the \textless think\textgreater  tag. We also conducted an additional MER task training using AvaMERG to facilitate the generation of accurate empathetic responses.

%  Finally, we fine-tune the entire architecture on a carefully balanced mixture of all tasks to unlock the model's full potential(see \cref{fig:P2E}, Phase 3). This involves activating a LoRA module for language model and is designed to cultivate synergies across tasks, from deepening fine-grained perception (OV-MER task) to eliciting high-level empathy (ERG task). Crucially, for ERG task, We use the Chain-of-Empathy~\cite{zhang2025towards} to guide the model to first consider the context of the conversation, the emotions of the interlocutor, and the goal of the response, thereby better generating empathetic responses.. To further ground the model's empathetic responses, we additionally define a standard emotion recognition sub-task on the AvaMERG dataset, helping the model to master the correlation between emotion and dialogue. A low sampling rate for MIR(5\%) is maintained to mitigate catastrophic forgetting. The data curriculum is a carefully balanced mixture with a sampling ratio of MER:OV-MER:MIR:ERI:ERG = 18:28:5:31:18.

% For the ERI task, we employed both the MER-Caption+~\cite{lian2025affectgpt} dataset and the meticulously annotated MERR-Fine~\cite{cheng2024emotion} to enhance the explanatory capabilities of the modal. We used the MIntRec~\cite{MIntRec} and MIntRec2.0~\cite{zhang2024mintrec} datasets to For the MIR, which are specifically designed for this task in conversational contexts, guiding the model to recognize fine-grained social goals and attitudes.

==> sec/4_exp.tex <==
\section{Experimental Analysis}
\label{sec:experiment}
%--------------------------------MER-UNIBENCH TAB---------------------------------------
\begin{table*}[t]
\centering
\footnotesize  % 缩小表格内文字大小
\caption{Performance comparison of different scale models on the MSA, MER and fine-grained OV-MER tasks. \textbf{AffectGPT (s)} marked with a $\dagger$ are trained solely on the MER-caption+ dataset, as proposed in the original work~\cite{lian2025affectgpt}. The best performance is displayed in \textbf{bold}, the second-best performance is \underline{underlined}.}
\label{tab:mer-unibench}
\renewcommand{\arraystretch}{0.95}  % 压缩行高


\resizebox{\linewidth}{!}{%
\begin{tabular}{@{\hspace{1pt}} c @{\hspace{2pt}} l@{\hspace{2pt}} *{10}{c} @{\hspace{1pt}}}
\toprule
Models & Scale & MER2023~\cite{lian2023mer} & MER2024~\cite{lian2024mer} & MELD~\cite{poria2018meld} & IEMOCAP~\cite{busso2008iemocap} & MOSI~\cite{zadeh2016mosi}& MOSEI~\cite{zadeh2018multimodal}& SIMS~\cite{yu2020ch}& SIMSV2~\cite{liu2022make}& OV-MERD~\cite{lian2025ovmer}& Avg. \\
\midrule
& & \multicolumn{4}{c}{\cellcolor{purple!20}Hit Rate $\uparrow$ (MER)} & \multicolumn{4}{c}{\cellcolor{green!10}WAF $\uparrow$ (MSA)} & {\cellcolor{blue!10}WAF $\uparrow$ (OV-MER)}& - \\
\midrule
SALMONN~\cite{tang2023salmonn} & \textcolor{Maroon}{$\uparrow$ 11.7B} & 55.53 & 45.38 & 45.62 & 46.84 & 81.00 & 67.03 & 68.69 & 68.69 & 45.00 & 57.89 \\
PandaGPT~\cite{su2023pandagpt} & \textcolor{Maroon}{$\uparrow$ 12.13B} & 40.21 & 51.89 & 37.88 & 44.04 & 61.92 & 67.61 & 68.38 & 67.23 & 37.12 & 52.92 \\
Mplug-Owl~\cite{ye2023mplug} & \textcolor{Maroon}{$\uparrow$ 5B} & 56.86 & 59.89 & 49.11 & 55.54 & 72.40 & 72.91 & 72.13 & 75.00 & 48.18 & 62.45 \\
Emotion-LLaMA~\cite{cheng2024emotion} & \textcolor{Maroon}{$\uparrow$ 5.6B} & 59.38 & 73.62 & 46.76 & 55.47 & 66.13 & 67.66 & 78.32 & 77.23 & 52.97 & 64.17 \\
AffectGPT~\cite{lian2025affectgpt} & \textcolor{Maroon}{$\uparrow$ 6.1B} & \underline{78.54} & \textbf{78.80} & \underline{55.65} & \textbf{60.54} & \textbf{81.30} & \textbf{80.90} & \textbf{88.49} & \textbf{86.18} & 62.52 & \textbf{74.77} \\
\midrule
\rowcolor{gray!30} \multicolumn{12}{c}{Small-scale Multimodal Models} \\
MobileVLM V2-1.7B~\cite{chu2024mobilevlm} & \textcolor{OliveGreen}{$\downarrow$ 0.5B} & 36.65 & 47.03 &  33.37 & 49.24 & 41.00 & 56.49 & 51.46 & 51.94 & 36.96 & 44.90 \\
MobileVLM V2-3B~\cite{chu2024mobilevlm} & \textcolor{Maroon}{$\uparrow$ 0.8B} & 37.70 & 53.87 &  30.72 & 53.00 & 55.81 & 44.87 & 69.17 & 65.72 & 33.86 & 49.95 \\
R1-Omni~\cite{zhao2025r1} & \textcolor{OliveGreen}{$\downarrow$ 0.1B} & 58.30 & 69.41 & 40.87 & 50.18 & 55.56 & 48.62 & 74.71 & 76.67 & 51.84 & 58.46 \\
AffectGPT (s)$^\dagger$ & \textcolor{OliveGreen}{$\downarrow$ 0.1B} & 73.45 & 74.71 & 47.69 & 53.14 & 75.51 & 71.30 & 82.50 & 84.10 & 62.43 & 69.43 \\
AffectGPT (s) & \textcolor{OliveGreen}{$\downarrow$ 0.1B} & 72.43 & 77.83 & 50.19 & 57.64 & \underline{80.40} & \underline{79.97} & 83.28 & 83.23 & \underline{63.75} & 72.08 \\
\midrule
\textbf{Our Nano EmoX} & 2.2B & \textbf{79.09} & 77.94 & \textbf{56.55} & \underline{60.12} & 76.82 & 79.81 & \underline{86.25} & \underline{84.76} & \textbf{64.75} & \underline{74.01} \\
\bottomrule
\end{tabular}%
}
\end{table*}
%--------------------------------MER-UNIBENCH TAB---------------------------------------
In this section, we conduct a series of experiments to analyze the multitask processing capabilities of Nano EmoX and the performance gains of the P2E framework. We perform evaluations on the benchmarks: MER-UniBench~\cite{lian2025affectgpt}, EMER~\cite{lian2023explainable}, MIntRec~\cite{MIntRec}, MIntRec 2.0~\cite{zhang2024mintrec} and AvaMERG~\cite{zhang2025towards}, where the evaluation metrics follow the official protocols. Refer to the appendix for detailed information on the benchmarks and evaluation metrics.

\subsection{Implementation Details}
\textbf{Model:} Nano EmoX uses CLIP-Large~\cite{radford2021learning} as visual encoder, HuBert-Large~\cite{hsu2021hubert} as speech encoder and Qwen 2.5-1.5B~\cite{qwen2025qwen25technicalreport} as LM, the token lengths for the visual, speech, facial and fusion streams are set to 32, 32, 4 and 1, respectively.
Additionally, to investigate the performance of a small-scale model, we constructed a controlled baseline, termed AffectGPT (s). This model is based on the AffectGPT, but replaces its original LLM with the more compact Qwen2.5-1.5B. To ensure a fair and direct comparison, AffectGPT (s) was trained using the identical P2E framework as Nano EmoX.

\textbf{Training details:} We used AdamW~\cite{loshchilov2019decoupled} as the training optimizer, with a consistent batch size of 3 and gradient accumulation steps of 4, and trained the model on a single NVIDIA RTX 4090 for 32 hours. The phase-specific hyperparameters for the P2E framework are as follows: 

\textbf{Phase 1}, The learning rate for all adapters was set to 3e-4. The visual/facial branches were trained for 25,000 steps and the speech branch for 15,000 steps.

 \textbf{Phase 2}, The learning rate for all trainable components was reduced to 1e-5, with training conducted for 5,000 steps.
 
 \textbf{Phase 3}, A uniform learning rate of 8e-6 was applied for the 300,000 step training. To conserve memory, the LoRA parameters were set with a $r$ of 32 and an $\alpha$ of 16.

\subsection{Performance Comparison}
\subsubsection{Zero-shot Evaluation on The MSA, MER and OV-MER Task}
To evaluate the intrinsic multimodal understanding capabilities of the model forged by our P2E framework, we first assess its zero-shot performance on benchmarks without any task-specific fine-tuning. As shown in \cref{tab:mer-unibench}, Nano EmoX's overall average score approaches the current SOTA results, with a mere 1.01\% performance gap despite a parameter reduction of approximately 70\%. Furthermore, our model establishes a new SOTA on both the coarse-grained emotion recognition benchmark MER2023, MELD and the fine-grained benchmark OV-MERD. This indicates that mixed-type adapters and fine-grained facial modeling within our audio-visual branch effectively promote the learning of diverse emotional expression styles and enhance overall affective generalization.

Notably, AffectGPT (s) trained with our P2E strategy exhibits a 2.65 percentage point performance increase over the specialist AffectGPT (s), which was trained with its original and richer dataset~\cite{lian2025affectgpt}. This experiment validates the facilitative role of the data curriculum employed in the P2E framework to enhance the model's emotion-aware capabilities.

\subsubsection{Zero-shot Evaluation on The ERI Task}
In the EMER challenge reason inference benchmark, as detailed in \cref{tab:emer}, our model achieves competitive performance. It surpasses numerous smaller models and even larger-scale methods, such as Video-LLaMA, PandaGPT and Valley. Moreover, it performs on par with Emotin-LLaMA while having significantly fewer parameters. This result underscores Nano EmoX's proficiency in capturing subtle, context-dependent emotional cues within dynamic conversations, thereby validating the effectiveness of our architectural design for temporal reasoning and contextual understanding.
%--------------------------------EMER TAB---------------------------------------
\begin{table}[t]  
\centering
\footnotesize  
\caption{Performance comparison of models of different scales on the task of ERI. Clue overlap measures the similarity between interpretable reasoning clues and real reasoning. The accuracy of emotion recognition of the model is evaluated by the Label overlap metric.}
\label{tab:emer}

\renewcommand{\arraystretch}{1.1}
\setlength{\tabcolsep}{3.1pt}
\begin{tabular}{c l c c}  % 无竖线，列格式为居中对齐
\toprule  % 顶部粗线
Models & Scale & Clue Overlap $\uparrow$ & Label Overlap $\uparrow$ \\
\midrule  % 中间细线
Video-LLaMA~\cite{zhang2023video} & \textcolor{Maroon}{$\uparrow$ 7.1B} & 6.64 & 4.89 \\
PandaGPT~\cite{su2023pandagpt} & \textcolor{Maroon}{$\uparrow$ 12.13B} & 7.14 & 5.51 \\
Valley~\cite{luo2023valley} & \textcolor{Maroon}{$\uparrow$ 6.04B} & 7.24 & 5.77 \\
Emotion-LLaMA~\cite{cheng2024emotion} & \textcolor{Maroon}{$\uparrow$ 5.6B} & 7.83 & 6.25 \\
Omni-Emotion~\cite{yang2025omni} & \textcolor{Maroon}{$\uparrow$ 6.8B} & \underline{8.22} & \underline{6.78} \\
Emotion-Qwen~\cite{huang2025emotion} & \textcolor{Maroon}{$\uparrow$ 5.3B} & \textbf{8.25} & \textbf{8.16} \\
\midrule 
\rowcolor{gray!30} \multicolumn{4}{c}{Small-scale Multimodal Models} \\ 
MobileVLM V2-1.7B~\cite{chu2024mobilevlm} & \textcolor{OliveGreen}{$\downarrow$ 0.5B} & 6.59 & 4.66 \\
MobileVLM V2-3B~\cite{chu2024mobilevlm} & \textcolor{Maroon}{$\uparrow$ 0.8B} & 6.49 & 4.82 \\
R1-Omni~\cite{zhao2025r1} & \textcolor{OliveGreen}{$\downarrow$ 0.1B} & 7.11 & 5.54 \\
AffectGPT (s) & \textcolor{OliveGreen}{$\downarrow$ 0.1B} & \underline{7.60} & \underline{5.70} \\
\midrule
\textbf{Our Nano EmoX} & 2.2B & \textbf{7.83} & \textbf{5.78} \\
\bottomrule 
\end{tabular}
\end{table}
%--------------------------------EMER TAB---------------------------------------
\subsubsection{Fine-Tuning Evaluation on The MIR Task}
\cref{tab:MIntrec} reveals that Nano EmoX exhibits competitive performance in fine-grained intent recognition, achieving best results among small-scale models with WF1 and WP scores of 58.17 and 60.12, respectively. Furthermore, the model surpasses a strong baseline, GPT-4o, on MIntRec 2.0 by 5 percentage points in accuracy (Acc) and 3.67 percentage points in WF1. These results underscore the potential of Nano EmoX for discriminating fine-grained intents.

However, in terms of overall performance, a gap remains when compared to larger-scale models in distinguishing subtle social intents. This is attributed to the difficulty of Nano EmoX's visual and facial branches in processing some high-resolution frame samples within MIntRec and MIntRec2.0, leading to the omission of valuable emotional cues. In future work, we will focus on enhancing Nano EmoX's performance on such high-resolution samples.
%--------------------------------MIntrec TAB---------------------------------------
\begin{table}[t]
\centering
\footnotesize
\caption{The evaluation results of the model in the multimodal intent recognition task. \textbf{Humans} represents the human performance from~\cite{MIntRec,zhang2024mintrec} report.}
\label{tab:MIntrec}

\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{2.5pt}

% 移除第二列后为7列，均居中对齐
\begin{tabular}{c c c c c c c}
\toprule  % 顶部粗线
Methods & \multicolumn{3}{c}{MIntRec} & \multicolumn{3}{c}{MIntRec 2.0} \\  
\cmidrule(lr){2-4} \cmidrule(lr){5-7}  % 子列分隔线调整为新列索引（原3-5→2-4，原6-8→5-7）
& Acc $\uparrow$ & WF1 $\uparrow$& WP $\uparrow$ & Acc $\uparrow$ & WF1 $\uparrow$ & WP $\uparrow$ \\ 
\midrule  % 中间主线
GPT-4 (zero shot)~\cite{achiam2023gpt} & 63.37 & 63.68 & 69.69 & 42.32 & 43.60 & 52.98 \\  
LLaVA-Video-72B~\cite{lin2023video} & 80.22 & 79.94 & 80.63 & 64.98 & 64.72 & 65.40 \\  
Qwen-VL-72B~\cite{wang2024qwen2} & \textbf{86.29} & \textbf{86.09} & \textbf{86.75} & \underline{66.99} & \underline{66.63} & \underline{67.45}\\  
MiniCPM-V-2.6-8B~\cite{hu2024minicpm} & 80.67 & 80.56 & 82.19 & 53.58 & 51.91 & 61.66 \\  
Qwen-2VL-7B~\cite{wang2024qwen2} & 82.92 & \underline{82.79} & \underline{86.75} & 64.19 & 63.31 & 64.39 \\  
Humans & \underline{85.51} & - & - & \textbf{71.03} & \textbf{75.63} & \textbf{81.83} \\  
\midrule 
\rowcolor{gray!30} \multicolumn{7}{c}{Small-scale Multimodal Models} \\ 
MAG-BERT~\cite{MIntRec,zhang2024mintrec} & 72.65 & - & - & 60.58 & 59.68 & 59.98 \\  
MUIT~\cite{MIntRec,zhang2024mintrec} & 72.52 & - & - & 60.66 & 59.55 & 60.12 \\ 
MobileVLM V2-1.7B~\cite{chu2024mobilevlm} & 33.27 & 33.81 & 34.75 & 21.34 & 22.64 & 25.59 \\  
MobileVLM V2-3B~\cite{chu2024mobilevlm} & 36.12 & 37.74 & 35.12 & 23.98 & 24.16 & 26.45 \\    
AffectGPT (s) & 48.76 & 50.71 & 57.87 & 38.79 & 37.18 & 41.91 \\  
\midrule 
\textbf{Our Nano EmoX} & 58.20 & 58.17 & 60.12 & 47.32 & 47.27 & 51.10 \\  
\bottomrule  % 底部粗线
\end{tabular}

% 恢复默认列间距
\setlength{\tabcolsep}{6pt}
\end{table}
%-----------------------------avamerg tab-----------------------------------------------
\begin{table}[t]
\centering
\footnotesize  
\caption{Performance comparison of models of different scales on the task of ERG. MiniCPM-o-2.6B~\cite{hu2024minicpm}, Qwen2.5-Omni-7B~\cite{xu2025qwen2}, Ola-Omni-7B~\cite{liu2025ola} all enhanced their capabilities by using the E3RG~\cite{lin2025e3rg}method.}
\label{tab:Avamerg}

% 调整行间距，保持紧凑性
\renewcommand{\arraystretch}{1.05}
\setlength{\tabcolsep}{6.3pt}

% 删除第二列后为4列，均居中对齐
\begin{tabular}{c c c c}
\toprule  % 顶部粗线
Models & Acc / Hit Rate $\uparrow$ & Dist-1 $\uparrow$ & Dist-2 $\uparrow$ \\  
\midrule  % 中间主线
Empatheia~\cite{zhang2025towards} & 48.51 / - & 2.69 & 14.76 \\  
MiniCPM-o-2.6B~\cite{hu2024minicpm} & - / 65.8 & 95.20 & 99.60 \\  
Qwen2.5-Omni-7B~\cite{xu2025qwen2} & - / 72.3 & 98.60 & 99.70 \\  
Ola-Omni-7B~\cite{liu2025ola} & - / 75.6 & 98.90 & 99.80 \\  
\midrule  
\rowcolor{gray!30} \multicolumn{4}{c}{Small-scale Multimodal Models} \\
CEM~\cite{sabour2022cem} & 37.32 / - & 0.50 & 2.07 \\  
CASE~\cite{zhou2022case} & 40.96 / - & 0.54 & 2.14 \\
MobileVLM V2-1.7B~\cite{chu2024mobilevlm} & 4.07 / 21.14 & 75.07 & 96.91 \\
MobileVLM V2-3B~\cite{chu2024mobilevlm} & 25.18 / 61.42 & 78.66 & 97.41 \\ 
AffectGPT (s) & \underline{47.36} / \underline{90.88} & \underline{95.44} & \textbf{99.81} \\ 
\midrule
\textbf{Our Nano EmoX} & \textbf{54.82 / 91.13} & \textbf{95.47} & \underline{99.73} \\  
\bottomrule  % 底部粗线
\end{tabular}

\setlength{\tabcolsep}{6pt}
\end{table}
%-----------------------------avamerg tab-----------------------------------------------
\subsubsection{Fine-Tuning Evaluation on The ERG Task}
On the ERG task, our model continues to demonstrate superior performance. As detailed in \cref{tab:Avamerg}, Nano EmoX achieves an accuracy of 54.82 in recognizing the speaker's emotion prior to generating an empathetic response, surpassing all other small-scale models. Notably, it sets a new SOTA in coarse-grained emotion recognition with a Hit Rate of 91.13, marking a 20.54 percentage point improvement over the previous SOTA method. Concurrently, AffectGPT (s), after being trained with P2E, achieves the second-best performance with a Hit Rate of 90.88. This validates the effectiveness of our cross-modal fusion encoder and the P2E framework for high-quality empathetic generation, highlighting our approach as a promising solution for enabling models to master rich, multi-layered knowledge.


%-----------------------------ablation evaluation----------------------------------------
\subsection{Ablation Evaluation}
\subsubsection{Modality Contribution Analysis}
To dissect our model's architectural contributions, we conducted a series of ablation studies detailed in \cref{tab:modality_contribution}. The bimodal variants serve as strong baselines but falter on the complex Empathic Response Generation task, underscoring the need for a more holistic perceptual system. Indeed, augmenting the visual stream with our dedicated Facial Perception Stream yields substantial performance gains, confirming the critical role of fine-grained facial cues that general-purpose encoders often miss.

The full Nano EmoX model significantly outperforms all partial configurations, demonstrating a powerful synergistic effect from integrating all perceptual streams. The efficacy of our specific design choices is further validated by two critical experiments. First, replacing our multiscale facial encoder with extracting 2D landmarks and face action units results in inferior performance. Second and most crucially, removing our hierarchical, gated fusion encoder entirely leads to a pronounced performance drop of 28.93 on AvaMERG, unequivocally proving its effectiveness in dynamically and efficiently integrating the multimodal streams.
%--------------------------------qualitative analysis fig--------------------------------
\begin{figure*}[t] % [t]表示优先放在页面顶部（跨双栏仅支持t/b位置）
    \centering
    \includegraphics[width=1.0\textwidth]{images/qualitative_analysis.pdf} % 替换为实际图片路径
    \caption{Qualitative results on the OV-MER, MIR, ERI and ERG task. Our model responds rapidly when handling perceptual tasks, while for interactive tasks, it first considers the interlocutor’s state before generating empathetic responses.}
    \label{fig:qualitative_analysis}
\end{figure*}
%--------------------------------qualitative analysis fig--------------------------------
%-------------------------------ablation branch tab--------------------------------------------
\begin{table}[t]
\centering
\footnotesize  % CVPR表格默认小字体
\caption{The influence of different branches combinations of Nano EmoX on performance was explored on the MER-UniBench~\cite{lian2025affectgpt}, EMER~\cite{lian2023explainable} and AvaMERG~\cite{zhang2025towards} benchmarks. `M' denotes the modality used by the model, where `A, V, F, M, T' represent Audio, Vision, Face, Fusion and Text modalities, respectively.}
\label{tab:modality_contribution}
\setlength{\tabcolsep}{1pt}

\begin{tabular}{c c c c c}
\toprule  % 顶部粗线
\multirow{2}{*}{Methods} & \multirow{2}{*}{M} & MER-Unibench & EMER & AvaMERG \\
\cmidrule{3-5}  % 仅分隔第3-5列
& & Avg. $\uparrow$ & Avg. $\uparrow$ & Hit Rate $\uparrow$ \\
\midrule  % 中间细线
Only Audio Branch         & AT    & 69.23 & 5.86 & 76.50 \\
Only Visual Branch        & VT    & 64.13 & 5.78 & 53.36 \\
Only Face Branch          & FT    & 65.99 & 5.63 & 46.54 \\
Visual + Face Branch & VFT   & 67.26 & 5.94 & 82.61 \\
w/o Fusion Branch     & AVFT  & 71.65 & 6.05 & 62.20 \\
W Face Landmark + AU     & AVFMT & 70.88 & 6.13 & 57.25 \\
w Fusion Branch       & AVFMT & \textbf{74.01} & \textbf{6.80} & \textbf{91.13} \\
\bottomrule  % 底部粗线
\end{tabular}
\setlength{\tabcolsep}{6pt} 

\end{table}

\subsubsection{Investigating Performance Improvements of The P2E Framework on Affective Tasks}

To isolate the contribution of our core training methodology, we compared the full P2E framework against an alternative training scheme: a standard Multitask Learning (MTL) setup where all tasks are trained jointly without our hierarchical curriculum and differentiated cognitive pathways.

The results, presented in \cref{tab:ablation_training}, are stark. While the standard MTL approach provides a solid foundation, particularly in perceptual tasks within MER-UniBench, our training method consistently outperforms it across all task categories. The most pronounced improvements are observed in the ERG task on the AvaMERG benchmark. After P2E training, the Hit Rate of AffectGPT (s) surged by an impressive 67.72\%, while Nano EmoX's increased by 17.93\%. This powerfully corroborates the efficacy of the P2E framework in deepening emotional perception and cultivating a more comprehensive form of emotional intelligence.

%-------------------------------ablation train method--------------------------------------------
\begin{table}[t]
\centering
\footnotesize
\caption{Comparison of training time cost and performance improvement results for different training methods.}
\label{tab:ablation_training}

% 压缩列间距以适配单栏宽度
\setlength{\tabcolsep}{2.2pt}

\begin{tabular}{c c c c c c}
\toprule  % 顶部粗线
\multirow{2}{*}{Models} & \multirow{2}{*}{Strategy} & \multirow{2}{*}{Time $\downarrow$} & MER-Unibench & EMER & AvaMERG \\
\cmidrule{4-6}  % 仅分隔第3-5列的子表头
& & & Avg. $\uparrow$ & Avg. $\uparrow$ & Hit Rate $\uparrow$ \\
\midrule  % 中间细线
AffectGPT (s) & MTL & 40 hours & 72.26 & 6.71 & 29.33 \\
Nano EmoX & MTL & 40 hours &73.28 & 6.54 & 74.79 \\
AffectGPT (s) & P2E &32 hours& 72.08 & 6.65 & 90.88 \\
\textbf{Nano EmoX} & P2E &32 hours& \textbf{74.01} & \textbf{6.76} & \textbf{91.13} \\
\bottomrule  % 底部粗线
\end{tabular}

% 恢复默认列间距（避免影响后续表格）
\setlength{\tabcolsep}{6pt}
\end{table}


\subsection{Qualitative Analysis on Nano EmoX}
%---------------------------------------qualitative-----------------------------------------
% \begin{figure}[t] % [t]表示优先放在当前栏顶部（单栏支持t/b/h等位置）
%     \centering
%     \includegraphics[width=1.1\columnwidth]{images/qualitative_analysis.pdf} % 用\columnwidth匹配单栏宽度
%     \caption{Qualitative results on four tasks: open vocabulary multimodal emotion recognition, multimodal intent recognition, Emotional Reason Inference and Empathetic Response Generation.}
%     \label{fig:qualitative analyze}
% \end{figure}
\cref{fig:qualitative_analysis} shows the visualization results of Nano EmoX on four key tasks. In the OV-MER task, our method can identify more fine-grained emotions of tension and anxiety. In the ERI task, Nano EmoX achieves accurate gender recognition compared to meticulously labeled ground-truth labels. Furthermore, in terms of the ERG task, after deliberative thinking, Nano EmoX generates more contextually appropriate responses.
%---------------------------------------qualitative analysis-----------------------------------------



